Aligning by Misaligning: Boundary-aware Curriculum Learning for Multimodal Alignment

Most multimodal models treat every negative pair alike, ignoring the ambiguous negatives that differ from the positive by only a small detail. We propose Boundary-Aware Curriculum with Local Attention (BACL), a lightweight add-on that turns these borderline cases into a curriculum signal. A Boundary-aware Negative Sampler gradually raises difficulty, while a Contrastive Local Attention loss highlights where the mismatch occurs. The two modules are fully differentiable and work with any off-the-shelf dual encoder. Theory predicts a fast O(1/n) error rate; practice shows up to +32% R@1 over CLIP and new SOTA on four large-scale benchmarks, all without extra labels.

==> sec/old-tables.tex <==
\begin{table}[tb]
  \centering
  \caption{Quantitative comparison against the other state-of-the-art methods on Mip-NeRF 360 dataset~\cite{barron2022mipnerf360}. We evaluate PSNR, SSIM, and LPIPS on 12 training views. Each training image is randomly chosen.}
  \resizebox{0.8\linewidth}{!}{%
  \small % Reduce the font size
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Model & Venue & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
        NeuS~\cite{wang2021neus}          & NeurIPS'21 & 18.7452 & 0.4951 & 0.4683 \\
    NeuralAngelo~\cite{li2023neuralangelo}                      & CVPR'23   & 18.5231 & 0.4827 & 0.4661 \\
    3DGS~\cite{kerbl3Dgaussians}         & TG'23   & 15.1386 & 0.4031 & 0.5593 \\
    SparseGS~\cite{xiong2023sparsegs}     & arxiv'23 & 15.9341 & 0.4188 & 0.4606 \\
    Dngaussian~\cite{li2024dngaussian}   & CVPR'24  & 15.6623 & 0.4120 & 0.4774 \\
    MatSparse3D~\cite{mao2024generating}  & CVPR'24  & 15.9450 & 0.4087 & 0.4653 \\
    CoR-Gs~\cite{zhang2025cor}   & ECCV'24 & \underline{19.3456} & \underline{0.5221} & 0.4373      \\
    FSGs~\cite{zhu2025fsgs}     & ECCV'24 & 18.4317 & 0.5084 & \underline{0.4492 }     \\
    InstantSplat~\cite{fan2024instantsplat} & arXiv'24  & 17.8962 & 0.4635 & 0.4785 \\
    SuGar~\cite{guedon2024sugar} & CVPR'24   & 19.0182 & 0.5104 & 0.4556 \\
    %2DGS                              & SIGGRAPH'24 & 18.9183 & 0.4982 & 0.4602 \\
    VCR-GauS~\cite{chen2024vcr}                         & NeurIPS'24  & 19.2113 & 0.5147 & 0.4534 \\
    PGSR~\cite{chen2024pgsr}                              & TVCG'24  & 19.1679 & 0.5073 & 0.4519 \\
    \midrule
    Ours         & -        & \textbf{19.9475} & \textbf{0.5642} & \textbf{0.4209} \\
    \bottomrule
  \end{tabular}
  }

\label{tab:MIP_quantitative}

\end{table}



\begin{table}[tb]
  \centering
  \caption{Quantitative comparison against the other state-of-the-art methods on the DTU dataset~\cite{DTU}. We evaluate both novel view synthesis (PSNR) and reconstructed mesh quality (Chamfer Distance) on 20 to 40 percent of the training images. Each training image is randomly chosen. The best values are highlighted in \textbf{bold}, and the second-best values are \underline{underlined}.}
  \resizebox{0.8\linewidth}{!}{%
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    Ratio (Used/All) & \multicolumn{2}{c}{$\alpha=0.2$} & \multicolumn{2}{c}{$\alpha=0.3$} & \multicolumn{2}{c}{$\alpha=0.4$} \\
    Metrics         & PSNR $\uparrow$ & CD $\downarrow$ & PSNR $\uparrow$ & CD$\downarrow$     & PSNR $\uparrow$ & CD $\downarrow$     \\
    \midrule
    MVSNeRF~\cite{chen2021mvsnerf}         & 22.65     & 7.53                 & 23.77     & 5.67                 & 23.85     & 5.23                 \\
    Mip-NeRF 360~\cite{barron2022mip}    & 24.86     & 4.28                 & 25.23     & 4.26                 & \underline{26.94}    & 4.35                 \\
    SparseNeuS~\cite{long2022sparseneus}      & 23.90     & \underline{3.70}     & 24.35     & \underline{3.21}     & 25.82    & \underline{3.14}     \\
    SparseNeRF~\cite{wang2023sparsenerf}      & 24.12     & 4.81                 & 25.44     & 4.07                 & 25.83     & 3.29                 \\
    3DGS~\cite{kerbl3Dgaussians}           & 22.14     & 5.64                 & 23.31     & 3.39                 & 24.64    & 3.29                 \\
    SparseGS~\cite{xiong2023sparsegs}        & 25.23    & 4.42                 & \underline{26.19}     & 3.45                 & 26.56    & 3.71                 \\
    Dngaussian~\cite{li2024dngaussian}       & 24.61     & 4.12                 & 24.89     & 4.36                 & 25.33    & 3.99                 \\
    MatSparse3D~\cite{mao2024generating}     & \underline{25.75}     & 5.49                 & 25.86     & 4.64                 & 25.99    & 4.23                 \\
InstantSplat~\cite{fan2024instantsplat}                         & 23.10 & 4.12 & 24.23 & 3.90 & 25.37 & 3.85 \\
      NeuS~\cite{wang2021neus}              & 23.72 & 4.50 & 24.55 & 3.98 & 25.49 & 3.67 \\
      NeuralAngelo~\cite{li2023neuralangelo}                         &  24.10 & 4.30 & 25.12 & 3.80 & 26.20 & 3.50 \\
      SuGar~\cite{guedon2024sugar}                                   & 24.80 & 4.20 & 25.48 & 3.60 & 26.55 & 3.44 \\
      2DGS~\cite{huang20242d}                                 & 24.70 & 4.22 & 25.30 & 3.64 & 26.22 & 3.55 \\
      VCR-GauS~\cite{chen2024vcr}        & 25.02 & 4.18 & 25.90 & 3.50 & 26.70 & 3.40 \\
      PGSR~\cite{chen2024pgsr}                                & 25.05 & 4.16 & 25.85 & 3.48 & 26.64 & 3.42 \\
      \midrule
    
    
    Ours            & \textbf{27.05}     & \textbf{3.49}         & \textbf{27.38}     & \textbf{3.07}         & \textbf{27.89}     & \textbf{3.01}  \\ 
    \bottomrule
  \end{tabular}
  }
  
  \label{tab:DTU_quantitative}
\end{table}
